On the Query Strategies for Efficient Online Active Distillation

Deep Learning (DL) requires lots of time and data, resulting in high computational demands. Recently, researchers employ Active Learning (AL) and online distillation to enhance training efficiency and real-time model adaptation. This paper evaluates a set of query strategies to achieve the best training results. It focuses on Human Pose Estimation (HPE) applications, assessing the impact of selected frames during training using two approaches: a classical offline method and a online evaluation through a continual learning approach employing knowledge distillation, on a popular state-of-the-art HPE dataset. The paper demonstrates the possibility of enabling training at the edge lightweight models, adapting them effectively to new contexts in real-time.

==> src/methodology_old.tex <==
%\subsection{Sampling methods}

% \begin{figure*}[t]
% \centering
% %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% \includegraphics[width=\linewidth]{fig/fig2.pdf}
% \caption{Timeline}
% \label{fig:timeline}
% \end{figure*}


% \mirco{
% Concepts to present in methodology: (1) definition of \emph{no sampling}, \emph{fixed-rate}, \emph{rate-free} metrics; (2) formal properties of \emph{fixed-rate} and \emph{rate-free} metrics; (3) formal definition and descriptive definition of each proposed metric (which are: uniform, random, svd/frequency, oracle/mpjpe, minconfidence, meanconfidence);}


%Example of a formal definition of a sampling method. Let $X$, the set of the samples collected during the continual learning process of size $N$, be defined as $X = \{ s_0, s_1, s_2, ..., s_j, ..., s_{N-1}\}$, where $s_j$ is a sample of index $i$ in the collection queue (TODO: queue to be defined). 
% \noindent Properties for rate-free metrics: 
% \begin{enumerate}
%     \item $0 < \lvert free\_sampling(X) \rvert < N$
%     \item while model performance keeps good, no train is performed
%     \item $free\_sampling(X) \stackrel{\propto}{\sim}  best\_sampling(X)$
%     \item ...
% \end{enumerate}
% Metric descriptive definition: The uniform sampling is defined as a function that takes in input the set of samples $X$ and the percentage $p$ of samples to extrapolate and gives ... 
% Metric formal definition: $uniform(X, p) = \{ s_j \in X \mid i \bmod 1 / p = 0 \}$

% Mirco here
The aim of active learning is to iteratively select the most informative data samples for annotation, thereby reducing the labeling effort while maintaining or improving the performance of the model. To achieve this we explore four sampling metrics used for fine-tuning a human pose estimation model: uniform, random, confidence and oracle sampling. Let $D$ be the a set of samples, defined as the $D = \{ s_0, s_1, ..., s_j, ..., s_N \}$, where $N$ is the total amount of frames of the dataset. A sampling strategy $\mathcal{S}$ is a function that selects a subset $D' \subseteq D$ based on a specific criterion or rule. Formally, $\mathcal{S}: Set[D] \rightarrow Set[D]$, where $Set[D]$ is a set of $D$ elements, such that $D' = \mathcal{S}(D)$, where $D'$ represents the selected subset of samples.

The sampling metrics employed in this study are implemented as fixed-rate strategies, where they operate by selecting a specific percentage of frames within a defined window of samples. Given the initial training dataset $D$, defined as the $D = \{ s_0, s_1, ..., s_j, ..., s_N \}$, where $N$ is the total amount of frames of the training-set, the sampling metrics is applied to each element of the set $D_{windowing} = \{ w_0, w_1, ..., w_i, ..., w_M \}$ where $M = \ceil*{N / W}$, $W$ is the size of the window and $w_i = \{s_j \mid M * i <= j <= M * (i+1) \}$. A fixed-rate sampling select, with a certain metric, a portion of the window of the indicated percentage. Then, given a window $w_i \subset D$ and a percentage $p \in P$, a fixed-rate sampling metric is defined as $fixed\_sampling: (Set[D], P) \rightarrow Set[D]$, where $D$ is the dataset as previously defined and $P = \mathbb{R}_{[0,1]}$. 

% The following are the properties of a fixed-rate sampling: (1) $fixed\_sampling(w_i, p) \subseteq w_i$; (2) $\lvert fixed\_sampling(w_i, p) \rvert = \lvert w_i \rvert * p$; (3) $\{ s_j\in D \mid \exists w_i \in D_{windowing},  s_j \in fixed\_sampling(w_i, p) \} \not\equiv fixed\_sampling(D, p)$; (4) $fixed\_sampling(w_i, 1) \equiv w_i$ and $fixed\_sampling(w_i, 0) \equiv \emptyset$. The properties 1 and 2 establish that fixed-sampling involves extracting a subset of the original input set of samples, where the size of the resulting set is determined by a percentage that corresponds to the specified proportion of the initial set's cardinality. The property 3 clarifies that when applying sampling to a dataset with a defined window, the outcome may not be identical to applying sampling directly to the entire dataset. Finally, property 4 emphasises that if you apply sampling at percentage 1, then you get no-sampling, with percentage 0 instead you get empty set. 
The fixed-sampling involves extracting a subset of the original input set of samples, where the size of the resulting set is determined by a percentage that corresponds to the specified proportion of the initial set's cardinality. When applying sampling to a dataset with a defined window, the outcome may not be identical to applying sampling directly to the entire dataset. Then if you apply sampling at percentage 1, then you get no-sampling, with percentage 0 instead you get empty set. 


The implemented sampling metrics in this study all utilize fixed-rate sampling. The following will provide definitions for each of the sampling metrics: uniform sampling, random sampling, confidence sampling, and oracle sampling.

%Uniform sampling is a straightforward approach where data samples are selected uniformly from the dataset with a specific rate that is inferred from the input percentage: $rate=1/p$. It does not take into account any specific criteria or model information and treats all unlabeled samples equally. Similarly to the $fixed\_sampling(w, p)$ function, the uniform sampling is defined as a function that takes in input the set of window samples $w$ and the percentage $p$ of samples to extrapolate and gives $uniform\_sampling(w, p) = \{ s_j \in w \mid i \bmod 1 / p = 0 \}$.
%Similar to uniform sampling, random sampling selects data samples randomly from the dataset. However, it can differ from uniform sampling in terms of the randomization process employed. While uniform sampling may utilize a deterministic randomization technique, random sampling can use more sophisticated randomization methods, such as stratified random sampling, to ensure a more representative selection of samples. As previously, the random sampling is defined as a function that takes in input the set $w$ and the percentage $p$ and gives $random\_sampling(w, p) = \{ s_j \in sort(random(w), \floor{W*p}) \}$, where $random(w, n)$ is a function, defined as $random: Set[D] \rightarrow Set[D]$, that randomly select the samples in the input set $w$ and $sort(w, n)$ is a function, defined as $sort: (Set[D], \mathbb{N}^+) \rightarrow Set[D]$, that sort the input set $w$ by the index $j$ of the samples $s_j \in w$ in ascending order and takes the first $n$ input samples.
%Confidence sampling aims to select data samples based on the model's confidence in its predictions. For human pose estimation, this metric can be determined by calculating the uncertainty or confidence score associated with each sample. Samples with high uncertainty or low confidence are considered more informative and are prioritized for annotation, as they are likely to be challenging or ambiguous cases for the model. The confidence sampling is defined as a function that takes in input the set $w$ and the percentage $p$ and gives $confidence\_sampling(w, p) = \{ s_j \in sort(confidence(w), \floor{W*p}) \}$, where $confidence(w)$ is a function, defined as $confidence: Set[D] \rightarrow Set[\mathbb{R}_{[0,1]}]$, that gives the mean-per-joint confidence of the samples and $sort(w, n)$ is the function as previously defined.
%Oracle Sampling is a sampling metric that selects frames with the highest error, specifically the Mean Per Joint Position Error (MPJPE), in comparison to a ground truth. It leverages the ground truth annotations to identify the frames where the model's predictions deviate the most from the true pose. By selecting these challenging frames, Oracle Sampling aims to provide the model with the most informative examples for improving its performance. The oracle sampling is defined as a function that takes in input the set $w$ and the percentage $p$ and gives $oracle\_sampling(w, p) = \{ s_j \in sort\_descending(mpjpe(w, gt), \floor{W*p}) \}$. The $mpjpe(w, gt)$ is a function, defined as $mpjpe: (Set[D], Set[GT]) \rightarrow Set[\mathbb{R}]$, that gives the MPJPE error between the input samples $w$ and the ground truth $gt \in GT$ with $GT$ the set of ground-truths of the dataset $D$. The function $sort\_descending(w, n)$ is the same of $sort$ but in descending order.

Uniform sampling selects data samples uniformly from the dataset with a rate determined by $rate=1/p$. Random sampling, similar to uniform, selects samples randomly but may use more sophisticated randomization methods. Confidence sampling selects samples based on the model's confidence in predictions, prioritizing uncertain or low-confidence cases. Oracle sampling selects frames with the highest error, MPJPE, compared to ground truth, aiming to provide challenging examples for model improvement.


%\fakepar{11-15}




% \begin{algorithm}[h]
% \caption{Efficient online distillation}\label{alg:two}
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \SetKwFunction{Inference}{inference}
% \SetKwFunction{GetImage}{getImage}
% \SetKwFunction{Train}{train}
% \Input{$\text{NN}_s$, $\text{NN}_t$}
% \Output{res}
% \While{$true$}{
% $I_i = $\GetImage{}\\
% res $ = $ \Inference{$I_i, \text{NN}_s$}
% }
% \end{algorithm}



